Uncertainty Quantification in Deep Residual Neural Networks

Uncertainty quantification is an important and challenging problem in deep learning. Previous methods rely on dropout layers which are not present in modern deep architectures or batch normalization which is sensitive to batch sizes. In this work, we address the problem of uncertainty quantification in deep residual networks by using a regularization technique called stochastic depth. We show that training residual networks using stochastic depth can be interpreted as a variational approximation to the intractable posterior over the weights in Bayesian neural networks. We demonstrate that by sampling from a distribution of residual networks with varying depth and shared weights, meaningful uncertainty estimates can be obtained. Moreover, compared to the original formulation of residual networks, our method produces well-calibrated softmax probabilities with only minor changes to the network's structure. We evaluate our approach on popular computer vision datasets and measure the quality of uncertainty estimates. We also test the robustness to domain shift and show that our method is able to express higher predictive uncertainty on out-of-distribution samples. Finally, we demonstrate how the proposed approach could be used to obtain uncertainty estimates in facial verification applications.

==> sections/Discussion.tex <==
We proposed a novel approach for obtaining uncertainty estimates in deep residual neural network. We showed that our approach produces meaningful uncertainty estimates and can be implemented with little effort.

%Limitations!
% Depth
% No fine granularity
% Tuning of hyper-oparameters

Despite the effectiveness of our method there are some limitations. The first being that the approach can only be applied to architectures with skip connections.  Another shortcoming is the fact that shorter networks are more susceptible to dropping out a large amount of residual blocks than deeper ones. Because there is less capacity for redundancy among the residual blocks than in a very deep network. Obtaining "fine grained" uncertainty estimates in shorter networks might be  requires perhaps deeper networks with more residual units.

Another shortcoming  with stochasticity, requires longer training times because the weight are inactive for a long period of training time. The deeper the network becomes the more possibilities/configurations there are.

Further research has to be done on the optimal drop rate for each residual block. One possibility is to learn the hyper-parameter during the training process.


% Discuss the strengths and weaknesses of your approach, based on the results. Point out the implications of your novel idea on the application concerned.
